Dielectrowetting of a thin nematic liquid crystal layer

We consider a mathematical model that describes the flow of a Nematic Liquid Crystal (NLC) film placed on a flat substrate, across which a spatially-varying electric potential is applied. Due to their polar nature, NLC molecules interact with the (nonuniform) electric field generated, leading to instability of a flat film. Implementation of the long wave scaling leads to a partial differential equation that predicts the subsequent time evolution of the thin film. This equation is coupled to a boundary value problem that describes the interaction between the local molecular orientation of the NLC (the director field) and the electric potential. We investigate numerically the behavior of an initially flat film for a range of film heights and surface anchoring conditions.

==> bibliography.tex <==
% This is the bibtex file for dielectrowetting-draft.tex

@ARTICLE{Brown2009,
	author={Brown, C.V. and Wells, G.G. and Newton, M.I. and McHale, G.},
	title={Voltage-programmable liquid optical interface},
	journal={Nature Photonics},
	year={2009},
	volume={3},
	number={7},
	pages={403-405},
	doi={10.1038/nphoton.2009.99}
	}

@article{McHale2011,
	title = {Dielectrowetting Driven Spreading of Droplets},
	author = {McHale, G. and Brown, C. V. and Newton, M. I. and Wells, G. G. and Sampara, N.},
	journal = {Phys. Rev. Lett.},
	volume = {107},
	issue = {18},
	pages = {186101},
	numpages = {4},
	year = {2011},
	doi = {10.1103/PhysRevLett.107.186101}
}

@ARTICLE{Edwards2018,
	author={Edwards, A.M.J. and Brown, C.V. and Newton, M.I. and McHale, G.},
	title={Dielectrowetting: The past, present and future},
	journal={Current Opinion in Colloid and Interface Science},
	year={2018},
	volume={36},
	pages={28-36},
	doi={10.1016/j.cocis.2017.11.005}
	}
	
@ARTICLE{SIAM_ODE15s,
    author = {Shampine, L. F. and Reichelt, M. W.},
title = {The MATLAB ODE Suite},
journal = {SIAM J. Sci. Comput.},
year = {1997},
volume = {18},
number = {1},
issn = {1064-8275},
doi = {10.1137/S1064827594276424},
pages = {1–22},
numpages = {22}
}
 
     
@article{chenjing,
        author={Cummings,L. J. and Cai,C. and Kondic,L.},
        year={2013},
        title={Towards an optimal model for a bistable nematic liquid crystal display device},
        journal={J. Eng. Math.},
        volume={80},
        number={1},
        pages={21-38},
        issn={0022-0833},
	doi={10.1007/s10665-012-9607-4},
 }    
@article{gliding,
        title = {Gliding of liquid crystals on soft polymer surfaces},
  	author = {J\'anossy,I. and K\'osa,T. I.},
  	journal = {Phys. Rev. E},
  	volume = {70},
  	issue = {5},
  	pages = {052701},
  	numpages = {4},
  	year = {2004},
}    
@article{nonuniform_field,
	author={Cummings,L. J. and Mema,E. and Cai,C. and Kondic,L.},
	title={Electric-field variations within a nematic-liquid-crystal layer},
	journal={Phys. Rev. E},
	year={2014},
	volume={90},
	number={1},
	pages = {012503},
}     
@book{DeGennes1995,
	address = {New York, NY},
	author = {De Gennes,P. G. and Prost,J.},
	publisher = {Oxford University Press},
	title = {{The physics of liquid crystals}},
	year = {1995},
}        
@article{Rapini,
	author = {Rapini,A. and Papoular,M.},
	journal = {J. Phys. Colloq. (Paris)},
	pages = {54},
	title = {{Distorsion d'une lamelle nematique sous champ magnetique, conditions d'ancrage aux parois}},
	volume = {30},
	year = {1969},
}
@book{Chandrasekhar,
	address = {Cambridge, UK},
	author={{Chandrasekhar},S.},
	publisher={Cambridge University Press},
	title={{Liquid Crystals}},
	year = {2007},
}
@article{DurandandVirga,
	author={Durand,G. E. and Virga,E. G.},
	year={1999},
	title={Hydrodynamic model for surface nematic viscosity},
	journal={Phys. Rev. E},
	volume={59},
	number={4},
	pages={4137-4142},
}
@book{Optics,
	address={Hoboken, NJ},
	author={Yeh,P. and Gu,C.},
	publisher={Wiley},
	title={{Optics of Liquid Crystal Displays}},
	year = {2009},
}
@article{Vetter&Ohmura,
	author={Vetter,P. and Ohmura,Y. and Uchida,T.},
	year={1993},
	title={Study of memory alignment of nematic liquid crystals on polyvinyl alcohol coatings},
	journal={Jpn. J. Appl. Phys, Part 2: Letters},
	volume={32},
	number={9A},
	pages={L1239-L1241},
}
@article{azimuth_gliding,
	author={Vorflusev,V. P. and Kitzerow,H.  and Chigrinov,V. G.},
	year={1997},
	title={Azimuthal surface gliding of a nematic liquid crystal},
	journal={Appl. Phys. Lett.},
	volume={70},
	number={25},
	pages={3359-3361},
}
@article{Faetti,
	author={Faetti,S. and Nobili,M. and Raggi,I.},
	year={1999},
	title={Surface reorientation dynamics of nematic liquid crystals},
	journal={Eur. Phys. J. B},
	volume={11},
	number={3},
	pages={445-453},
}
@article{Davidson,
	author={Davidson,A. J. and Mottram,N. J.},
	year={2002},
	title={Flexoelectric switching in a bistable nematic device},
	journal={Phys. Rev. E},
	volume={65},
	number={5},
	pages={051710},
}
@article{Richardson,
	author={Cummings,L. J. and Richardson,G.},
	year={2006},
	title={Bistable nematic liquid crystal device with flexoelectric switching},
	journal={Eur. J. Appl. Math},
	volume={17},
	number={4},
	pages={435-463},
}
@book{stewart,
	address={London, UK},
	author={{Stewart},I. W.},
	publisher={Taylor \& Francis},
	title={{The Static and Dynamic Continuum Theory of Liquid Crystals.}},
	year = {2004},
}
@article{Leslie,
	author={Leslie,F. M. },
	year={1979},
	title={Theory of flow phenomena in liquid crystals.},
	journal={Adv. Liq. Cryst.},
	volume={4},
	number={},
	pages={1-81},
}
@article{Kedney&Leslie,
	author={Kedney,P. J. and  Leslie,F. M.},
	year={1998},
	title={Switching in a simple bistable nematic cell. },
	journal={Liq. Cryst.},
	volume={24},
	number={4},
	pages={ 613-618},
}
@article{flex_disp,
	author={},
	year={2011},
	title={Advances in Display Technologies; and E-Papers and Flexible Displays.},
	journal={Proc. SPIE Conf.},
	volume={7956},
	number={4},
	pages={ 613-618},
}
@ARTICLE{Pasechnik2006175,
	author={Pasechnik,S. V. and Chigrinov,V. G. and Shmeliova,D. V. and Tsvetkov,V. A. and Kremenetsky,V. N. and Zhijian,L. and Dubtsov,A. V.},
	title={Slow relaxation processes in nematic liquid crystals at weak surface anchoring},
	journal={Liq. Cryst.},
	volume={33},
	number={2},
	pages={175-185},
	year = {2006},
}
@article{Joly,
	author={Joly,S. and Antonova,K. and Martinot-Lagarde,P. and Dozov,I.},
	title={Zenithal gliding of the easy axis of a nematic liquid crystal},
	journal={Phys. Rev. E},
	year={2004},
	volume={70},
	number={51},
	pages={050701},
}
@article{Choi2008581,
	author = {Choi,M. C. and Kim,Y. and Ha,C. S.},
	year = {2008},
	title = {Polymers for flexible displays: From material selection to device applications},
	journal = {Prog. Poly. Sci.},
	volume = {33},
	number = {6},
	pages = {581-630},
}
@ARTICLE{Janossy2005,
	author={J\'anossy,I.},
	title={High-precision measurement of azimuthal rotation of liquid crystals on solid substrates},
	journal={J. App. Phys.},
	year={2005},
	volume={98},
	number={4},
	pages={043523},
}
@article{Yokoyama_top,
	author={Gwag,J. S. and Kim,J. -H. and Yoneya,M. and Yokoyama,H.},
	year={2008},
	title={Surface nematic bistability at nanoimprinted topography},
	journal={Appl. Phys. Lett.},
	volume={92},
	number={15},
	pages={153110},
}
@article{PhysicsToday,
	author={Palffy-Muhoray,P.},
	year={2007},
	title={The diverse world of liquid crystals},
	journal={Phys. Today},
	volume={60},
	number={9},
	pages={54-60},
}
@article{Meyer,
	author={Meyer,R. B.},
	title={Piezoelectric effects in liquid crystals},
	journal={Phys. Rev. Lett.},
	year={1969},
	volume={22},
	number={18},
	pages={918-921},
}
@article{daCosta,
	author={Da Costa,F. P. and Grinfeld,M. and Mottram,N. J. and Pinto,J. T.},
	title={Uniqueness in the {F}reedericksz transition with weak anchoring},
	journal={J. Differ. Equations},
	year={2009},
	volume={246},
	number={7},
	pages={2590-2600},
}
@ARTICLE{Derzhanski,
	author={Derzhanski,A. and Petrov,A. G. and Mitov,M. D.},
	title={One-dimensional dielectric-flexoelectric defomations in nematic layers},
	journal={J. Phys. (Paris)},
	year={1978},
	volume={39},
	number={3},
	pages={273-285},
}
@ARTICLE{Napoli,
	author={Napoli,G.},
	title={Weak anchoring effects in electrically driven {F}reedericksz transitions},
	journal={J.  Phys. A: Mathematical and General},
	year={2006},
	volume={39},
	number={1},
	pages={11-31},
}
@BOOK{Yang,
	author={{Yang},D. -K. and Wu,S. -T.},
	title = {Fundamentals of Liquid Crystal Devices},
 	year = {2006},
 	publisher = {John Wiley \& Sons},
}
@book{Buka,
	address = {London, UK},
	author = {{Buka},A. and \'Eber,N.},
	publisher = {Imperial College Press},
	title = {{Flexoelectricity in Liquid Crystals: Theory, Experiments and Applications}},
	year = {2013},
}
@book{Blinov_Chigrinov,
	address = {New York, NY},
	author = {Blinov,L. M. and Chigrinov,V.},
	publisher = {Springer},
	title = {{Electrooptic Effects in Liquid Crystal Materials}},
	year = {1994},
}	
@ARTICLE{Freedericksz_tr,
	author={{Fr\'eedericksz},V. and Repiewa,A.},
	title={Theoretisches und Experimentelles zur Frage nach der Natur der anisotropen Fl\"ussigkeiten},
	journal={Z. Phys.},
	year={1927},
	volume={42},
	number={7},
	pages={532-546},
}
@BOOK{Pasechnik_book,
	author={Pasechnik,S. V. and Chigrinov,V. G. and Shmeliova,D. V.},
	title={Liquid Crystals: Viscous and Elastic Properties},
	publisher={Wiley-VCH},
	address={Weinheim, Germany},
	year={2009},
	pages={39-42},
}
@ARTICLE{Mema2015,
	author={Mema,E. and Kondic,L. and Cummings,L. J.},
	title={Substrate-induced gliding in a nematic liquid crystal layer},
	journal={Phys. Rev. E},
	year={2015},
	volume={92},
	number={6},
	pages={062513},
}
@ARTICLE{Cummings2013,
	author={Cummings,L. J. and Cai,C. and Kondic,L.},
	title={Bifurcation properties of nematic liquid crystals exposed to an electric field: Switchability, bistability, and multistability},
	journal={Phys. Rev. E},
	year={2013},
	volume={88},
	number={1},
	 pages = {012509},
}
@ARTICLE{Buluy,
	author={Buluy,O. and Iljin,A. and Ouskova,E. and Reznikov,Y. and Blanc,C. and Nobili,M. and Antonova,K.},
	title={Anchoring and gliding of easy axis of {5CB} on photoaligning {PVCN-F} surface},
	journal={J. Soc. Inf. Disp.},
	year={2006},
	volume={14},
	number={7},
	pages={603-610},
}
@ARTICLE{Kurioz,
	author={Kurioz,Y. and Reshetniak,V. and Reznikov,Y.},
	title={Orientation of a liquid crystal on a soft photoaligning surface},
	journal={Mol. Cryst. Liq. Cryst. Sci. Technol., Sect. A },
	year={2002},
	volume={375},
	pages={535-541},
}
@article{Palffy-Muhoray,
	author={Palffy-Muhoray,P.},
	title={The diverse world of liquid crystals},
	journal={Phys. Today},
	year={2007},
	volume={60},
	number={9},
	pages={54-60},
}
@article{TA_paper,
	author={Anderson,T. G. and Mema,E. and Kondic,L. and Cummings,L. J.},
	title={Transitions in Poiseuille flow of nematic liquid crystal},
	journal={Int. J. Nonlinear Mech. },	
	year={2015},
	volume={75},
	pages={15-21},
}
@article{ZBD_patent,
	author={Bryan-Brown,G. P. and Brown,C. V. and Jones,J. C.}, 
	title={Zenithal Bistable Device},
	journal={U.S. Patent 6249332},
	year = {1995},
 }
 @ARTICLE{PABD,
	author={Willman,E. and Fernandez,F. A. and James,R. and Day,S. E.},
	title={Switching dynamics of a post-aligned bistable nematic liquid crystal device},
	journal={J. Display Technol.},
	year={2008},
	volume={4},
	number={3},
	pages={276-281},
}
@ARTICLE{Ericksen1960,
	author={Ericksen,J. L.},
	title={Theory of Anisotropic Fluids},
	journal={J. Rheol.},
	year={1960},
	volume={4},
	number={1},
	pages={29-39},
}
@ARTICLE{Leslie1968,
	author={Leslie,F. M.},
	title={Some constitutive equations for liquid crystals},
	journal={Arch. Rational Mech. Anal.},
	year={1968},
	volume={28},
	number={4},
	pages={265-283},
}
@ARTICLE{Leslie1966,
	author={Leslie,F. M.},
	title={Some constitutive equations for anisotropic fluids},
	journal={Q. J. Mech. Appl. Math},
	year={1966},
	volume={19},
	number={3},
	pages={357-370},
}
@article{Brown2003,
	author={Brown,C. V. and Mottram,N. J.},
	title={Influence of flexoelectricity above the nematic {F}reedericksz transition},
	journal={Phys. Rev. E},
	year={2003},
	volume={68},
	number={31},
	pages={317021-317025},
}
@ARTICLE{Prost&Pershan,
	author={Prost,J. and Pershan,P. S.},
	title={Flexoelectricity in nematic and smectic-A liquid crystals},
	journal={J.  Appl. Phys.},
	year={1976},
	volume={47},
	number={6},
	pages={2298-2312},
}
@book{atkinson,
	  title={An Introduction to Numerical Analysis},
	  address={Hoboken, NJ},
	  author={Atkinson,K. E.},
	  year={1989},
	  publisher={Wiley},
}
@article {Lee2012,
	author = {Lee,J. -H. and Yoon,T. -H.},
	title = {P-77: Image Sticking in a Flexible Liquid Crystal Display Stabilized with Polymers: Surface Gliding Effect},
	journal = {{SID} Int. Sym. Dig. Tec.},
	year = {2012},
	volume = {43},
	number = {1},
	pages = {1343--1345},
}
@online{datathief,
  	title = {Data Thief {III}},
  	howpublished = "\url{http://datathief.org}",
	note="(Accessed on November 28, 2016)",
  	year="2015",
}
@online{di_coeff,
	howpublished="\url{http://www.mit.edu/~6.777/matprops/polyimide.htm}",
	note="(Accessed on November 28, 2016)",
}

@article{Faetti2006,
author={Faetti, S. and Marianelli, P.},
title={Azimuthal director gliding at a strongly anchoring interface of polyimide},
journal={Liq. Cryst.},
year={2006},
volume={33},
number={3},
pages={327-334},
}

@article{Oliveira1991,
author={Oliveira, E.A. and Figueiredo Neto, A.M. and Durand, G.},
title={Gliding anchoring of lyotropic nematic liquid crystals on amorphous glass surfaces},
journal={Phys. Rev. A},
year={1991},
volume={44},
number={2},
pages={R825-R827},
}

@ARTICLE{Antonova2011,
author={Antonova, K. and Slyusarenko, K. and Buluy, O. and Blanc, C. and Joly, S. and Reznikov, Y. and Nobili, M.},
title={Aging in glassy polymer-liquid-crystal layers},
journal={Phys. Rev. E},
year={2011},
volume={83},
number={5},
pages={050701},
}
